Revealing the Two Sides of Data Augmentation: An Asymmetric Distillation-based Win-Win Solution for Open-Set Recognition

In this paper, we reveal the two sides of data augmentation: enhancements in closed-set recognition correlate with a significant decrease in open-set recognition. Through empirical investigation, we find that multi-sample-based augmentations would contribute to reducing feature discrimination, thereby diminishing the open-set criteria. Although knowledge distillation could impair the feature via imitation, the mixed feature with ambiguous semantics hinders the distillation. To this end, we propose an asymmetric distillation framework by feeding teacher model extra raw data to enlarge the benefit of teacher. Moreover, a joint mutual information loss and a selective relabel strategy are utilized to alleviate the influence of hard mixed samples. Our method successfully mitigates the decline in open-set and outperforms SOTAs by 2%~3% AUROC on the Tiny-ImageNet dataset and experiments on large-scale dataset ImageNet-21K demonstrate the generalization of our method.

==> AnonymousSubmission/Figures/fig_ssl.tex <==
\begin{figure*}[!ht]
\centering
\scalebox{1}{
\includegraphics[width=1\linewidth]{AnonymousSubmission/Images/pipeline_ssl_final.pdf}}
\caption{
Teacher-free learning framework.
}
\label{fig:ssl}
\end{figure*}

==> AnonymousSubmission/Figures/fig_top2_error.tex <==
\begin{figure}[!ht]
\centering
\scalebox{1.0}{
\includegraphics[width=0.8\linewidth]{AnonymousSubmission/Images/teacher's_top2_4.pdf}}
\caption{The teacher's top-2 error rate and over-confident predictions (higher than 95\%) under different mixing coefficients. 
% When the samples are mixed averagely, the teacher will make more wrong predictions(about 15\%). 
% The teacher's over-confident predictions range from 20\% to 70\% which can not be overlooked during this procedure.
}
\label{fig:top2_error}
\end{figure}

==> AnonymousSubmission/Figures/fig_various_ratio.tex <==
\begin{figure}[!ht]
\centering
% 0.87
\includegraphics[width=0.7\linewidth]{AnonymousSubmission/Images/various_ratio.pdf}
\caption{
The performances under various $\lambda$ on Tiny-ImageNet dataset.
% With different fixed mixing coefficients, the model's AUROC and close-set accuracy vary too. The best performance appears when the samples are mixed average because the model can get more information within one CutMix sample. When the samples are mixed randomly, the model can meet various inputs for better Open-set competence.
}
\label{fig:various_ratio}
\end{figure}

==> IJCAI_2024/Sections/Cover_letter.tex <==
% \section{Cover Letter}
\section{Summary of the Reviews}
\begin{enumerate}
    \item This paper is written in rather poor English, making it hard to understand the analysis and technical contents.
    \item For SSA, only the CutOut is verified. It is hard to support that single-sample-based augmentation can improve the model's open-set performance.
    \item In Table~1, the readers would like to see how the distillation works on ResNet-50.
    % `when model is trained with single-sample-based augmentation, its open-set performance is enhanced'.
    \item The analyzing part of the paper lacks the concrete proof and the actual visualization about the changes in feature space.
    % The visualization part of the paper lacks the concrete proof. / I think it would be better if there is an actual visualization about the changes in feature space.
    \item Some related works about data-mix augmentation are not mentioned in the paper.
    \item The motivation of $\mathcal{L}_{CMI}$ and Two-hot Label Smoothing are both confusing (too many intuitive sentences with few references or formula derivation).
    \item The complexity of involving an additional teacher model.
    \item These types of work require testing on large-scale datasets such as ImageNet.
    % I am mainly concerned about the complexity of the paper proposal.
\end{enumerate}
\section{Modifications}
\begin{enumerate}
    \item We polish our descriptions and conduct in depth analysis using visualizations and formula derivations to enable the readers to understand both the insight and our method.
    \item To support our conclusion, we conducted experiments on more models and more data augmentation methods. For single-sample-based augmentation, we introduce AugMix~\cite{hendrycks2020augmix} and Randomized Quantization~\cite{wu2023randomized} to validate the positive impact of SSA on model's both open-set performance and close-set performance.
    \item The distillation experiments of ResNet-50 and ResNet-101 are conducted to demonstrate the impact of distillation on model's open-set performance.
    \item To interpret how multiple-sample-based augmentation influences the model's feature space, we visualize the changes of the feature norms for all individual classes in Section~3.2 of the main text. Further, we draw t-SNE visualizations on MNIST dataset in section~A of the supplementary material to get a more intuitive view of the changes in feature space. The comparisons of the activation magnitude of different models are also listed to explain how MSA and distillation influence the model.
    \item We state the difference between our method and previous open-set recognition works who consider the data-mix augmentation as the unknown samples in Section~1 of the main text. And we associate our experimental observation to the work which investigates the role of MixUp in the distillation~\cite{choi2023understanding}.
    \item To clarify the purpose of $\mathcal{L}_{CMI}$ and Two-hot Label Smoothing, we start from the analysis in Section~3 and conduct formula derivations to account for the role of the two terms in eliminating the degradation of open-set performance.
    \item The light-weight edition of our method is introduced in section~B of the supplementary material by removing the teacher network. The ablations of the teacher-free framework also validate the effectiveness of the two terms in our method.
    \item We test our method on ImageNet-21k dataset to prove the generalization of our method. Our method achieves the SOTA performance within the large-scale dataset. And we conduct the experiment of MobileNet-V2 to validate the improvement of our method on the light-weight models. 
\end{enumerate}
